Alignment and Comparison of Directed Networks via Transition Couplings of Random Walks

We describe and study a transport based procedure called NetOTC (network optimal transition coupling) for the comparison and alignment of two networks. The networks of interest may be directed or undirected, weighted or unweighted, and may have distinct vertex sets of different sizes. Given two networks and a cost function relating their vertices, NetOTC finds a transition coupling of their associated random walks having minimum expected cost. The minimizing cost quantifies the difference between the networks, while the optimal transport plan itself provides alignments of both the vertices and the edges of the two networks. Coupling of the full random walks, rather than their marginal distributions, ensures that NetOTC captures local and global information about the networks, and preserves edges. NetOTC has no free parameters, and does not rely on randomization. We investigate a number of theoretical properties of NetOTC and present experiments establishing its empirical performance.

==> GOTC-0_intro.tex <==

\section{Introduction}

Networks have long been used as a means of representing and studying the pairwise interactions between 
a set of individuals or objects under study.  More recently, networks themselves have become objects of
study.  Networks appear as data objects in a number of
applications, including comparing protein interaction networks \citep{Singh2008global, Kazemi2016PROPERGP, Kelley2004PathBLASTAT, Elmsallati2016GlobalAO}, aligning single-cell multi-omics data \citep{demetci2020gromov}, deanonymizing private networks \citep{narayanan2008robust, narayanan2009deanonymizing, Qian2016DeanonymizingSN}, pattern recognition \citep{Conte2004ThirtyYO, Bai2012GraphBasedMI, Lzoray2017ImagePA}, image captioning \citep{chen2020graph, Yao2018ExploringVR}, and language comparison \citep{alvarez2018gromov}.  

Analysis of network-based data often begins with network alignment or comparison, tasks that have been studied in a number of fields.
In the simplest version of the network alignment problem, one is given two networks with vertex sets of equal size and seeks to find a bijection between the vertex sets that maximizes the number of aligned edges.  
Numerous approaches to network alignment have been considered in the literature, e.g. \cite{Kelley2003ConservedPW, Kuchaiev2010TopologicalNA, Kuchaiev2011IntegrativeNA, Kalaev2008FastAA, Klau2009ANG}. 
By contrast, the goal of network comparison is to identify quantitative differences between weighted networks of different sizes or structures.  Networks of this sort may arise from distinct data sets or scientific domains.

In this paper, we propose and analyze Network Comparison and Alignment using Optimal Transition Coupling (NetOTC), 
a flexible procedure for the comparison and soft alignment of weighted networks that is based on a process-level 
version of optimal transport.   
The NetOTC procedure takes as input two connected networks $G_1$ and $G_2$ with non-negative edge weights, and a cost function 
relating their vertices.  
Each network gives rise to a random walk on its vertex set, which is a stationary Markov chain.  
NetOTC proceeds by finding a coupling of these Markov chains (a transport plan) that is itself stationary 
and Markov, and that minimizes the expected value of the cost function at any given time point.  
(For computational and theoretical reasons discussed below, 
NetOTC considers a sub-family of Markov couplings known as transition couplings.)
The optimal transport plan is a stationary random walk on the product of the vertex sets of the given networks that favors low cost pairs, while maintaining the marginal structure of the random walks on each individual network.

The cost function used in NetOTC is specified by the user, and will, in general, be application dependent.  
Cost functions can be based, for example, on the difference between externally specified vertex attributes, the distance between Euclidean embeddings of the vertices, and the difference between the degrees of the vertices.  If the given networks have the same vertex set, a cost function based on vertex identity may be used as well.


The NetOTC procedure has a number of desirable methodological and theoretical properties.
On the methodological side, NetOTC applies to directed and undirected networks, and readily handles networks with different sizes and 
connectivity structures.  
As NetOTC considers process-level couplings of random walks, the optimal transport plan
captures global information reflected in the stationary distributions of the random walks, 
as well as local information that is present in the transition probabilities between vertices. 
The expected cost of the optimal transport plan provides a numerical measure of the difference between the networks.  
The distribution of the optimal transport plan at a single time point yields a soft, probabilistic alignment of the vertices in the given networks.  
Moreover, the distribution of the optimal transport plan at two successive time points yields a soft, probabilistic alignment of the {\em edges} of the given networks.
To the best of our knowledge, native alignment of edges is unique to NetOTC among existing alignment and comparison methods.  
The exact version of the NetOTC procedure has no free parameters and is not randomized.  

On the theoretical side, we establish several key properties of the NetOTC procedure that support its use in comparison and alignment tasks.
The edge alignment of NetOTC respects edges, in the sense that vertex pairs in the given networks are aligned with positive probability 
only if each pair is connected by an edge in its respective network.
Although the NetOTC optimal transport plan minimizes the expected cost between vertices at a single time point,
stationarity ensures that the coupled random walk has a low average cost between vertices across time.
The NetOTC similarity measure is sensitive to differences in the $k$-step behavior of
the random walks on $G_1$ and $G_2$ if these differences affect the cumulative cost.  
For undirected networks with a common vertex set,
the NetOTC similarity is a metric on equivalence classes of networks 
having identical random walks if the cost $c$ is a metric.  
For the zero-one cost, the NetOTC similarity is lower bounded by the $L_1$-difference of the network 
degree sequences, and the $L_1$-difference of the network weight functions.

In addition, we study the structure of the NetOTC method through network factors.  
Our definition of factor, which arises naturally when considering functions of Markov chains, differs from other definitions in the network theory literature.
Informally, a network $G_2$ is a factor of a network $G_1$ if the vertices of $G_2$ can be associated, 
via a vertex map $f$, with disjoint
sets of vertices in $G_1$ between which aggregate weights can be consistently defined.
If $G_2$ is a factor of $G_1$ we show that the vertex map
$f$ yields a deterministic transition coupling of their associated random walks.
Under suitable compatibility conditions on the cost function, this coupling will be optimal and will provide a solution to the NetOTC problem.  
The resulting expected cost, vertex and edge alignments are fully determined by the structure of $G_1$ and the map $f$.
Importantly, the existence and precise nature of the map $f$ need not be known to the NetOTC procedure.
These results extend to paired factors: an optimal transition coupling for a pair of networks can be mapped in a deterministic fashion to an optimal transition coupling of their factors
when the cost functions for each pair are compatible with the factor maps.  

As a complement to the theory, we carry out a number of simulations and numerical experiments to assess the performance of NetOTC and compare it with other optimal transport-based comparison methods in the literature.  
NetOTC is competitive with other methods on a number of network classification tasks.
In an extensive experiment on pairs of isomorphic networks with small to moderate sizes, NetOTC was consistently able to recover the isomorphism using a local (degree-based) cost function, substantially outperforming other methods.
When applied to stochastic block models (with equivalent blocks of different sizes) using a degree-based cost function, NetOTC was competitive with other methods in its ability to align vertices in equivalent blocks, and substantially better at aligning edges.  
We also considered the problem of comparing a network to an exact or approximate factor using a distance-based cost derived from Euclidean vertex embeddings of the given networks.
NetOTC outperforms other methods in its ability to align vertices in the parent and factor networks.  While the performance gap is modest for exact factors, it increases as one considers approximate factors.

\subsection{Outline of the Paper}

The next section gives an overview of existing work on optimal transport and related approaches to network comparison and alignment.  Section \ref{sec:transition_couplings} 
provides background concerning random walks on directed networks, optimal transport for Markov chains, 
and transition couplings.  
The NetOTC procedure is described in Section \ref{sec:graphotc}, including 
computation, the optimal transport cost, and vertex and edge alignment.
Section \ref{sec:theory} is devoted to the formal statement and discussion of the theoretical properties of NetOTC.
Proofs are given in Section \ref{sec:proofs}.
Section \ref{sec:experiments} contains a number of simulations and a number of experiments that demonstrate the flexibility and potential utility of NetOTC. 
Additional details concerning the experiments are given in Appendix \ref{app:exp_details}. 


==> GOTC-0_rel-work.tex <==

\section{Related Work}
\label{sec:related_work}

\textcolor{red}{}

The problems of network alignment and comparison have received a lot of recent attention in the literature.  Approaches using optimal transport ideas can be divided into two groups: spectral and variants of Gromov-Wasserstein.  Other approaches make use of quadratic programming
and continuous approximations.  This related work is discussed below.

\paragraph{Spectral Methods.} 

One line of work \citep{dong2020copt, maretic2019got, maretic2020wasserstein} uses techniques from spectral graph theory to define optimal transport (OT) problems for networks.
In particular, this approach associates to each network a multivariate Gaussian with zero mean and covariance matrix equal to the pseudo-inverse of the graph Laplacian.
The Wasserstein distance between Gaussian distributions of the same dimension may be computed analytically 
in terms of their respective covariance matrices.
For networks with different numbers of vertices, \cite{maretic2020wasserstein} and \cite{dong2020copt} propose to optimize this distance over soft many-to-one assignments between vertices in either network.
At present, this family of approaches is unable to incorporate available feature information or underlying cost functions, relying only on their intrinsic structure.

\paragraph{Variants of Gromov-Wasserstein.}
Another line of work \citep{memoli2011gromov, peyre2016gromov, titouan2019optimal,vayer2019sliced,vayer2020fused} considers the Gromov-Wasserstein (GW) distance and related extensions.
In this work, one tries to couple distributions on the vertices in each network so as to minimize an expected transport cost between vertices while minimizing changes in edges between the two networks.
This approach allows one to capture differences in both features and structure between networks.
We refer the reader to \cite{dong2020copt} for a discussion on the differences between spectral-based network OT methods and GW distances.
A number of variants of the GW distance have been proposed for a variety of tasks including cross-domain alignment \citep{chen2020graph}, graph partitioning \citep{xu2019scalable}, graph matching \citep{xu2019scalable, xu2019gromov}, and node embedding \citep{xu2019gromov}.
The work \citep{barbe2020graph} proposes to incorporate global structure into the Wasserstein and Fused GW (FGW) distances by applying a heat diffusion to the vertex features before computing the cost matrix.

\paragraph{Other Methods for Network Alignment and Comparison.}
There is also a large body of work devoted to network alignment and comparison that do not use optimal transport methods.
The network alignment problem can be generally defined as a quadratic programming problem under discrete and doubly stochastic constraints \citep{yan2016ashort, jiang2017graph, loiola2007asurvey, cho2010reweighted, cour2007balanced}.
However, as the optimal network alignment problem is well known to be an NP-hard problem \citep{garey1990computers}, it is computationally challenging to obtain an optimal alignment for networks. 
For this reason, many authors have proposed approximate solutions for network alignment \citep{cho2010reweighted, zhou2016factorized, yu2018generalizing, enqvist2009optimal, van2004apocs, zaslavskiy2009apath}. 
Among these approximate methods, most of the successful algorithms start with relaxing the discrete constraints to create a continuous condition. Several authors
\citep{schellewald2005probabilistic, torr2003solving} relax the discrete conditions to form a positive semi-definite problem. A non-convex quadratic programming problem was adopted in \cite{gold1996agraduated, cho2010reweighted, zhou2016factorized}. In another direction, \cite{leordeanu2005aspectral} introduces spectral matching as a simple relaxation, and \cite{cour2007balanced} strengthens this approach by giving an affine constraint.
Also, \cite{jiang2017graph} proposes an algorithm that can efficiently solve a general quadratic programming problem with doubly stochastic constraints. Each step of the algorithm is easy to implement and the convergence is guaranteed. Generally, after finding the optimal solution for the relaxed continuous problem, the discrete alignment is attained through a final discretization process \citep{cho2010reweighted, leordeanu2005aspectral, leordeanu2009aninteger}.
We note that these approaches may find a solution that is locally optimal but not globally optimal.

There is also a line of research devoted to the statistical and probabilistic analysis of graph matching when the 
given graphs are generated at random but are correlated with one another, e.g., each is a random 
perturbation of a given graph \citep{Ding2020EfficientRG, Barak2019NearlyEA, Cullina2020PartialRO, Cullina2017ExactAR, Feizi2020SpectralAO, Korula2014AnER, Lyzinski2014SeededGM, Yartseva2013OnTP}. 
Much of this work investigates various matching procedures under specific random graph models, 
such as correlated Erdos-Renyi graphs,
and is concerned with the information-theoretic threshold for exact recovery, and the time complexity 
of the matching procedures.

==> GOTC-1_theory.tex <==

\section{Theoretical Properties of NetOTC}
\label{sec:theory}

In this section, we explore some theoretical properties of NetOTC, beginning 
with the edge-alignment property and several results concerning the behavior of NetOTC under average cost criteria.
For undirected networks with a common vertex set, we establish that the NetOTC cost has the properties of a metric 
when the cost $c$ does, and we investigate the sensitivity of NetOTC to local information arising from degree and 
weight functions.
We then define a notion of \textit{network factor} that captures the idea of one network being
``folded'' or ``compressed'' to produce another.  Although the literature contains several definitions of 
network factors or factor networks, the definition given here appears to be new.  We establish a 
close connection between factors and transition couplings, and then  we
present two results describing the behavior of NetOTC in the presence of this type of network factor structure.
All proofs of the results in this section may be found in Section \ref{sec:proofs}.


\subsection{NetOTC Edge Alignment}

The NetOTC edge alignment function $\pi_{\text{e}}$ respects edges, in the sense that vertex pairs aligned with 
positive probability must be adjacent in the given networks.

\begin{restatable}[]{prop}{edgepreservation}
\label{prop:edge_preservation}
Let $\pi_{\text{e}}$ be the NetOTC edge alignment of networks 
$G_1 = (U, E_1, w_1)$ and $G_2 = (V, E_2, w_2)$ based on the optimal transport plan $(X^*, Y^*)$.
If $\pi_{\text{e}}((u,u'),(v,v')) > 0$ then $(u,u') \in E_1$ and $(v,v') \in E_2$. 
\end{restatable}


\subsection{NetOTC and Multistep Cost}\label{sec:multistep_cost}

The NetOTC cost $\rho(G_1,G_2)$ is the expected cost
$\E c(\tilde{X}_0,\tilde{Y}_0)$ at the initial state of the optimal transport plan.   Here we consider
the average cost of the optimal transport plan over multiple time points, which provides
insights into the behavior of NetOTC.

\begin{defn}
For an infinite sequence $x_0, x_1, \ldots$ and integers $0 \leq i \leq j$ let $x_i^j = (x_i, \dots, x_j)$.  
For each $k \geq 1$ define the $k$-step average cost 
$c_k(x_0^{k-1}, y_0^{k-1}) = k^{-1} \sum_{j=0}^{k-1} c(x_j, y_j)$ and the limiting average cost
$\overline{c}(x,y) = \limsup_{k \to \infty} c_k(x_0^{k-1}, y_0^{k-1})$.
\end{defn}

Stationarity ensures that the NetOTC problem is equivalent to minimizing the 
long-term average cost over the set of transition couplings.

\begin{restatable}[]{prop}{gotceq}
\label{prop:gotceq}
Let $G_1$ and $G_2$ be networks with associated random walks $X$ and $Y$.
Then
\[
\rho(G_1, G_2) 
\ = \
\min_{(\tilde{X}, \tilde{Y}) \in \tc(X,Y)} \E \overline{c}(\tilde{X}, \tilde{Y}),
\]
and the optimal transport plans minimizing $\E \overline{c}(\tilde{X}, \tilde{Y})$ coincide with those
minimizing $\E c(\tilde{X}_0, \tilde{Y}_0)$.
\end{restatable}

The long-term behavior of the random walks $X$ and $Y$ encodes information about 
the global structure of the networks $G_1$ and $G_2$, respectively. 
The next result shows that NetOTC also captures local information arising from the finite time behavior 
of the walks $X$ and $Y$. 
For example, if $G_1$ and $G_2$ are distinguishable based on optimal transport of their $k$-step random walks, 
then they are distinguishable by NetOTC. 

\begin{restatable}[]{prop}{gotclowerbound}
\label{prop:gotclowerbound}
Let $G_1$ and $G_2$ be networks with associated random walks $X$ and $Y$.
For each $k \geq 1$
\[
\rho(G_1, G_2) 
\ \geq \ 
\min \ \E \, c_k(\tilde{X}_0^{k-1}, \tilde{Y}_0^{k-1}) ,
\]
where the minimum is over the family of all couplings of $X_0^{k-1}$ and $Y_0^{k-1}$.
\end{restatable}


\subsection{Undirected Networks with a Common Vertex Set}

In this section, we consider undirected networks $G_1 = (U, E_1, w_1)$ and $G_2 = (U, E_2, w_2)$ with the same vertex set,
but potentially different edge sets and weight functions.  We assume throughout that the networks are connected.
We begin by defining a natural equivalence relation on such networks.


\begin{defn}
Undirected networks $G_1$ and $G_2$ are
\emph{equivalent}, denoted by $G_1 \sim G_2$, if they have the same vertex $U$, the same edge set $E$, and there exists a constant 
$C > 0$ such that $w_1(u, u') = C \, w_2(u, u')$ for every $u, u' \in U$.
\end{defn}

The following result relates the equivalence of networks to their random walks. 

\begin{restatable}[]{prop}{graphequiv}
\label{prop:equiv}
Connected undirected networks $G_1$ and $G_2$ are equivalent 
if and only if their respective random walks are identical.
\end{restatable}

Whatever the underlying cost $c$, the cost $\rho(G_1,G_2)$ and optimal transport plan arising from 
NetOTC depend only on the equivalence classes of the networks $G_1$ and $G_2$.  In particular,
NetOTC is invariant under (positive) scaling of weight functions.  
When the underlying cost $c$ is a metric on $U$, the NetOTC cost is a metric on these equivalence classes.

\begin{restatable}[]{prop}{gotcismetric}
\label{prop:gotcismetric}
If the cost function $c: U \times U \rightarrow \mathbb{R}_+$ satisfies the properties of a metric on $U$,
then $\rho$ is a metric on the equivalence classes of undirected networks with vertex set contained in $U$ defined by $\sim$.
\end{restatable}


We now investigate the sensitivity of NetOTC to differences between the degree and weight functions
of the given networks.

\begin{defn}
The degree function of an undirected network $G = (U, E, w)$ is given by 
$d(u) = \sum_{u' \in U} w(u,u')$ for $u \in U$.  Let $D = \sum_{u \in U} d(u)$ denote the total degree of $G$.
\end{defn}

The next proposition strengthens the general result of Proposition \ref{prop:gotclowerbound}.

\begin{restatable}[]{prop}{lowerbound}
\label{prop:locallowerbound}
Let $G_1$ and $G_2$ be undirected networks with the same vertex set.  
Let $d_1(u)$ and $d_2(u)$ be the degree functions of $G_1$ and $G_2$, respectively, 
and assume that each network has total degree $D$. 
Then under the zero-one cost $c(u, u') = \In(u \neq u')$, 
\begin{itemize}
\item $\rho(G_1, G_2) \geq \frac{1}{2D} \sum\limits_{u \in U} |d_1(u) - d_2(u)|$
\item $\rho(G_1, G_2) \geq \frac{1}{4D} \sum\limits_{u, u' \in U} |w_1(u,u') - w_2(u,u')|$ 
\end{itemize}
\end{restatable}




\subsection{Deterministic Transition Couplings and Factor Maps}
\label{sec:factors}

The graph theory and network literature contain several definitions of ``network factor'' and ``factor network''. 
A network factor of $G$ is often defined to be any spanning subnetwork of $G$, while   
the term factor network is used in the context of message passing algorithms and error-correcting codes to refer to a 
bipartite network that captures the factorization of a function or a probability distribution.
Here we define a notion of network factor that appears to be different than existing definitions in the literature,
see for example the survey \citep{plummer2007graph}.
We show that there is a close connection between factors and transition couplings, and we use this to rigorously
study the behavior of NetOTC when factor structure is present.  Our results establish a close link between
NetOTC and factors, behavior that distinguishes NetOTC from other comparison and alignment methods.


\begin{defn}
\label{def:factor}
Let $G_1 = (U,E_1,w_1)$ and $G_2 = (V,E_2,w_2)$ be strongly connected, weighted directed networks with out-degree functions $d_1$ and $d_2$, respectively. 
A map $f : U \to V$ is  a \emph{factor map} if 
for all $v,v' \in V$ and $u \in f^{-1}(v)$, 
\begin{equation} \label{eq:factor_def}
\sum_{u' \in f^{-1}(v')} w_1(u,u') \ = \ \frac{d_1(u)}{d_2(v)} \, w_2(v,v').
\end{equation}
In this case, we will say that $G_2$ is a \emph{factor} of $G_1$, and that $G_1$ is an \emph{extension} of $G_2$.
\end{defn}


\begin{ex}\label{ex:factor1}
Consider the networks $G_1$ and $G_2$ drawn in Figure \ref{fig:factor_ex1} with vertices embedded in $\bbR^2$.
$G_2$ is a factor of $G_1$ with respect to the map $f$ that takes $(-1, 1)$ and $(-1, -1)$ to $(-1, 0)$, $(0, 0)$ to $(0, 0)$, and $(1, 0)$ and $(1, -1)$ to $(1, 0)$.
\end{ex}


The definition of factor arises naturally from the random walk perspective.  If $G_1$ and $G_2$ have associated
random walks $X$ and $Y$, and $G_2$ is a factor of $G_1$ under the map $f$, then the process 
$f(X) := f(X_1), f(X_2), \ldots$ is equal in distribution to $Y$, see 
Theorem \ref{thm:factortc} below for more details. 
Factors have been well studied in ergodic theory and symbolic dynamics.
The existence of a factor map (in the sense above) ensures that $Y$ is a stationary coding of $X$, which is a special case 
of a factor relationship in ergodic theory. 
Moreover, if $G_2$ is a factor of $G_1$, then the subshift of finite type (SFT) consisting of all bi-infinite walks on 
$G_2$ is a topological factor of the SFT associated with $G_1$ given by a $1$-block code
(see \cite{lind1995anintroductiontosymbolicdynamics} for detailed definitions). 
Our definition of factor has points of contact with compressed representations of weighted networks, 
explored in \cite{toivonen2011compression}, but in general the relationship \eqref{eq:factor_def} need not hold for compressed representations.  



\begin{figure}[t]
\centering
\begin{subfigure}{0.45\textwidth}
\centering
\scalebox{0.5}{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
                    thick,main node/.style={circle,draw,font=\sffamily\Large\bfseries}]

  \node[main node] (3) {(0,0)};
  \node[main node] (1) [above of=3, left of=3]{(-1,1)};
  \node[main node] (2) [left of=3, below of=3] {(-1,-1)};
  \node[main node] (4) [right of=3] {(1,0)};
  \node[main node] (5) [below of=4] {(1,-1)};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node[left] {1} (2)
    (2) edge (1)
    (2) edge [bend right] node[below] {1} (3)
    (3) edge [left] node[above, left] {1} (2)
    (3) edge [right] node[below, left] {1} (1)
    (1) edge [bend left] node[above] {1} (3)
    (3) edge [left] node[below] {1} (4)
    (4) edge [bend right] node[above] {1} (3)
    (3) edge [right] node[above, right] {1} (5)
    (5) edge [bend left] node[below] {1} (3)
    (4) edge node[right] {1} (5)
    (5) edge (4);
\end{tikzpicture}
}
\caption{$G_1$}
\label{fig:factor_ex1a}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\centering
\scalebox{0.5}{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
                    thick,main node/.style={circle,draw,font=\sffamily\Large\bfseries}]

  \node[main node] (3) {(0,0)};
  \node[main node] (1) [left of=3]{(-1,0)};
  \node[main node] (4) [right of=3] {(1,0)};

  \path[every node/.style={font=\sffamily\small}]
    (3) edge node[below] {2} (1)
    (1) edge (3)
    (3) edge node[below] {2} (4)
    (4) edge (3)
    (1) edge [loop left] node[left] {2} (1)
    (4) edge [loop right] node[right] {2} (4);
\end{tikzpicture}
}\vspace{5mm}
\caption{$G_2$}
\label{fig:factor_ex1b}
\end{subfigure}
\caption{An example of two networks related by a factor map. Here $G_2$ is a factor of $G_1$ via 
the map that collapses vertices along vertical lines.}
\label{fig:factor_ex1}
\end{figure}


The definition of factor formalizes the idea that $G_2$ (the factor) is a collapsed or 
compressed version of $G_1$ (the extension).
The factor map $f$ associates the vertices in $G_2$ with a partition of the vertices in $G_1$. 
Condition \eqref{eq:factor_def} ensures that the partitioning of the vertices is consistent 
with the transition probabilities of the random walk on $G_1$. 
If $\bP$ and $\bQ$ are the transition kernels for $G_1$ and $G_2$, then Condition \eqref{eq:factor_def} is equivalent to the statement that 
for all $v,v' \in V$ and $u \in f^{-1}(v)$, 
\begin{equation} \label{eq:factor_trans_probs}
\sum_{u' \in f^{-1}(v')} \bP( u' \mid u) = \bQ( v' \mid v).
\end{equation}
This is also equivalent to the condition $\mathbb{P}( f(X_1) = v' \mid X_0 = u) = \mathbb{P}( Y_1 = v' \mid Y_0 = v)$,
where $X$ and $Y$ are the random walks associated with $G_1$ and $G_2$.
Since $\bP$ and $\bQ$ are irreducible, Condition \eqref{eq:factor_def} implies that the (unique) stationary distributions 
$\bp$ on $G_1$ and $\bq$ on $G_2$ are such that
for all $v \in V$, 
\begin{equation} \label{eq:stat_dist_factor_def}
\sum_{u \in f^{-1}(v)} \bp(u) = \bq(v),
\end{equation}
which is equivalent to $f(X_1) \eqd Y_1$. 
The factor relationship can also be expressed in matrix form. If $f$ is a factor map from $G_1$ to $G_2$, 
then \eqref{eq:factor_def} is equivalent to the condition $\bP F = F \bQ$ where
$F \in \mathbb{R}^{U \times V}$ is defined by $F(u,v) = 1$ if $f(u) = v$ and $F(u,v) = 0$ otherwise. 
Furthermore equation \eqref{eq:stat_dist_factor_def} is equivalent to $\bp F = \bq$.

\vskip.05in

The next proposition establishes a close connection between transition couplings and factor maps. 
Let $G_1$ and $G_2$ be strongly connected, weighted directed networks with associated random walks $X$ and $Y$.  
Note that any stationary Markov coupling $(\tilde{X},\tilde{Y})$ of $X$ and $Y$ corresponds to a weighted, directed 
network $H$ with vertex set $W \subset U \times V$.
Let $\pi_U : U \times V \to U$ and $\pi_V : U \times V \to V$ be the natural projections onto the first and second coordinates, respectively.

\begin{restatable}[]{prop}{TCinTermsFactors}
If $(\tilde{X},\tilde{Y})$ is a stationary Markov coupling corresponding to a strongly connected network $H$ with vertex set $W$, 
then $(\tilde{X},\tilde{Y})$ is a transition coupling of $X$ and $Y$ if and only if the restriction of $\pi_U$ to $W$ is a factor map from 
$H$ to $G_1$ and the restriction of $\pi_V$ to $W$ is a factor map from $H$ to $G_2$. 
\end{restatable}

We next investigate connections between factors and deterministic transition couplings.
 
\begin{defn} \label{def:DetTC}
Suppose $G_1 = (U, E_1, w_1)$ and $G_2 = (V, E_2, w_2)$ are two strongly connected, weighted, directed networks with associated Markov chains $X$ and $Y$, respectively. A transition coupling $(\tilde{X},\tilde{Y})$ is said to be deterministic from $X$ to $Y$ if for each $u$ in $U$ there exists $v \in V$ such that $\mathbb{P}( \tilde{Y}_0 = v \mid \tilde{X}_0 = u) = 1$. 
\end{defn}
In optimal transport theory, deterministic couplings are associated with the so-called Monge problem, see \cite{Villani2008OptimalTO} for more context and discussion.
A deterministic coupling $(\tilde{X}, \tilde{Y})$ from $X$ to $Y$ is associated with a map $f : U \to V$, where $f(u)$ is the 
(necessarily unique) element $v \in V$ for which $\mathbb{P}( \tilde{Y}_0 = v \mid \tilde{X}_0 = u) = 1$.
In particular, $(\tilde{X},\tilde{Y}) \eqd (X,f(X))$.  
Moreover, as $G_2$ is strongly connected, $\mathbb{P}(Y_0 = v) > 0$ for each $v \in V$, and
the edge-alignment property (Proposition \ref{prop:edge_preservation}) ensures that $f$ is a surjective 
graph homomorphism from $G_1$ to $G_2$.



\begin{restatable}[]{thm}{factortc}
\label{thm:factortc}
Suppose $G_1$ and $G_2$ are strongly connected, weighted directed networks with associated random walks $X$ and $Y$, respectively. 
\begin{enumerate}
\item If $G_2$ is a factor of $G_1$ with factor map $f$, then
$Y \eqd f(X)$, and 
$(X,f(X))$ is a deterministic transition coupling from $X$ to $Y$.
\item If $(\tilde{X},\tilde{Y})$ is a deterministic transition coupling from $X$ to $Y$, then the induced map $f : U \to V$ is a factor map from $G_1$ to $G_2$.
\end{enumerate}
\end{restatable}




When $G_2$ is a factor of $G_1$ under $f$, Theorem \ref{thm:factortc} ensures that $(X,f(X))$ is a transition coupling of
their random walks.  If the cost function $c$ is such that $c(u,v)$ is minimized by $v = f(u)$ then, as the next result shows, 
this coupling is also optimal, and there is a deterministic solution to the NetOTC problem.

\begin{defn}
Let $f$ be a factor map from $G_1$ to $G_2$.  A cost function $c$ is {\em compatible} with $f$ if
$c(u,f(u)) \leq c(u,v)$ for each $u \in U$ and $v \in V$.
\end{defn}

One may verify that the cost compatibility condition is satisfied in Example \ref{ex:factor1} under a Euclidean metric cost.

\begin{restatable}[]{cor}{factor}
\label{cor:factor} Suppose $G_1$ and $G_2$ are strongly connected, weighted directed networks and $f$ is a factor map from $G_1$ to $G_2$. 
If $c$ is compatible with $f$ then $(X,f(X))$ is an OTC of $X$ and $Y$.
\end{restatable}

An example illustrating Corollary \ref{cor:factor} is given in Figure \ref{fig:factor}.
Corollary \ref{cor:factor} provides some insight into the structure of the NetOTC problem.
If $G_1$ and $G_2$ are related by a factor map $f: U \rightarrow V$, then $G_2$ is essentially a compressed version of the network $G_1$.
Corollary \ref{cor:factor} ensures that an optimal coupling of the random walks on $G_1$ and $G_2$ is obtained by running the random
walk on $G_1$ and mapping every state $u \in U$ in this chain to the corresponding state $f(u) \in V$.
In practice, the conclusion of Corollary \ref{cor:factor} approximately holds when the factor condition \eqref{eq:factor_def} 
approximately holds; the results of experiments involving exact and approximate factors are given in Section \ref{sec:graph_factors}.


\begin{figure}[t]
\begin{center}
\begin{subfigure}{0.31\linewidth}
\includegraphics[width=\linewidth, trim=3.2cm 2.5cm 2.5cm 1.5cm, clip]{figures/factor_G1.png}
\caption{$G_1$}
\end{subfigure}
\begin{subfigure}{0.31\linewidth}
\includegraphics[width=\linewidth, trim=3.2cm 2.5cm 2.5cm 1.5cm, clip]{figures/factor_G2.png}
\caption{$G_2$}
\end{subfigure}
\begin{subfigure}{0.34\linewidth}
\centering
\captionsetup{justification=centering}
\includegraphics[width=\linewidth, trim=1.4cm 0.5cm 0.2cm 0.5cm, clip]{figures/factor_alignment.png}
\caption{Vertex alignment of $G_1$ and $G_2$ from NetOTC.}
\label{fig:factor_gotc}
\end{subfigure}
\caption{An illustration of the relationship between factors and the NetOTC problem.
Under the conditions described in Corollary \ref{cor:factor}, the NetOTC problem aligns vertices according to the factor map relating the two networks.
In this example, $G_2$ is a factor of $G_1$. 
Figure \ref{fig:factor_gotc} illustrates the NetOTC vertex alignment, which is supported on pairs of the form $(u, f(u))$.}
\label{fig:factor}
\end{center}
\end{figure}

Under the conditions of Corollary \ref{cor:factor}, the NetOTC cost and associated vertex and edges alignments will have a special form. 
In particular, the NetOTC cost will satisfy $\rho(G_1,G_2) = \sum_{u \in U} c(u, f(u)) \bp(u)$
where $\bp$ is the stationary distribution of the random walk on $G_1$. 
Furthermore, $\pi_v(u,v) = \mathbb{I}(f(u) = v)$ and
$\pi_e((u,u'),(v,v')) = \mathbb{I}((f(u),f(u')) = (v,v'))$.
Note that, while the deterministic coupling appears as a solution of the NetOTC problem, the NetOTC algorithm itself 
makes no reference to, and does not require prior information about, the factor map $f$.
The next result provides further information about how NetOTC behaves in the presence of factor maps.



\begin{restatable}[]{thm}{twofactor}
\label{thm:two_factor}
Let $G_1$, $G_2$, $H_1$, and $H_2$ be networks with vertex sets $U$, $V$, $A$, and $B$, and associated 
Markov chains $X$, $Y$, $W$, and $Z$, respectively. 
Suppose that $f : U \to A$ and $g : V \to B$ are factor maps from $G_1$ to $H_1$ and $G_2$ to $H_2$, 
and that there are cost functions $c_{ext} : U \times V \to \mathbb{R}_+$ and $c : A \times B \to \mathbb{R}_+$ such that $c_{ext}(u, v) = c( f(u) , g(v))$. 
\begin{enumerate}
\item If $(\tilde{X}, \tilde{Y})$ is an optimal transition coupling of $X$ and $Y$ with respect to $c_{ext}$, then $(f(\tilde{X}), g(\tilde{Y}) )$ is an optimal transition coupling of $W$ and $Z$ with respect to $c$.

\vspace{2mm}

\item If $(\tilde{W},\tilde{Z})$ is an optimal transition coupling of $W$ and $Z$ with respect to $c$, then there exists an optimal transition coupling $(\tilde{X},\tilde{Y})$ of $X$ and $Y$ with respect to $c_{ext}$ such that $(f(\tilde{X}), f(\tilde{Y})) \eqd (\tilde{W},\tilde{Z})$.
\end{enumerate}
\end{restatable}

A simple illustration of Theorem \ref{thm:two_factor} is given in Figure \ref{fig:two_factor}.
For compatible cost functions, the theorem ensures that an optimal transport plan for the extensions $G_1$ and $G_2$
can be transferred through the maps $f$ and $g$ to an optimal transport plan for the factors $H_1$ and $H_2$; moreover,
every optimal transport plan for the factors can be obtained in this way. 
Thus NetOTC respects factor structure whenever factor structure is present: the NetOTC alignment of the 
extensions is consistent with the NetOTC alignment of the factors.
This is a fundamental property of the NetOTC procedure, in the sense that the operation of NetOTC on the 
extensions $G_1$ and $G_2$ makes no reference to, and requires no knowledge of,
the factor maps $f$ and $g$ or the factors $H_1$ and $H_2$.






\begin{figure}[t]
\centering
\includegraphics[width=0.95\textwidth, trim=0cm 0cm 0cm 0cm, clip]{figures/two_factor.png}
\caption{An illustration of Theorem \ref{thm:two_factor}. If $G_1$ and $H_1$, and $G_2$ and $H_2$ are related by factor maps $f$ and $g$, respectively, the NetOTC of $H_1$ and $H_2$ can be naturally induced by the NetOTC of $G_1$ and $G_2$ using the maps $f$ and $g$.}
\label{fig:two_factor}
\end{figure}




